Learn Your Scales: Towards Scale-Consistent Generative Novel View Synthesis

Conventional depth-free multi-view datasets are captured using a moving monocular camera without metric calibration. The scales of camera positions in this monocular setting are ambiguous. Previous methods have acknowledged scale ambiguity in multi-view data via various ad-hoc normalization pre-processing steps, but have not directly analyzed the effect of incorrect scene scales on their application. In this paper, we seek to understand and address the effect of scale ambiguity when used to train generative novel view synthesis methods (GNVS). In GNVS, new views of a scene or object can be minimally synthesized given a single image and are, thus, unconstrained, necessitating the use of generative methods. The generative nature of these models captures all aspects of uncertainty, including any uncertainty of scene scales, which act as nuisance variables for the task. We study the effect of scene scale ambiguity in GNVS when sampled from a single image by isolating its effect on the resulting models and, based on these intuitions, define new metrics that measure the scale inconsistency of generated views. We then propose a framework to estimate scene scales jointly with the GNVS model in an end-to-end fashion. Empirically, we show that our method reduces the scale inconsistency of generated views without the complexity or downsides of previous scale normalization methods. Further, we show that removing this ambiguity improves generated image quality of the resulting GNVS model.

==> figures/translation_exp.tex <==
\begin{figure}[h]
  \centering
   \includesvg[width=\linewidth]{figures/translation_exp.svg}
   \caption{
   \textbf{Additional examples for scale ambiguity in GNVS models.} A solid line depicts a visually distinctive edge across all views. We place a dashed line on the generated views at the edge where it originally was in the observed view. We also use an arrow to highlight the displacement of the edge between the observed view and each of the generated views.
   }
   \label{fig:trans-exp}
\end{figure}


==> macros.tex <==
\newcommand{\comment}[1]{\textcolor{blue}{\bf #1}}
\newcommand{\jason}[1]{\textcolor{blue}{\bf Jason: #1}}
\newcommand{\fereshteh}[1]{\textcolor{violet}{\bf Fereshteh: #1}}
\newcommand{\kosta}[1]{\textcolor{blue}{\bf #1}}
\newcommand{\marcus}[1]{\textcolor{orange}{Marcus: #1}}
\newcommand{\ttaa}[1]
{\textcolor{teal}{Tristan: #1}}
\newcommand{\reviewme}[1]{\textcolor{gray}{[#1]}}

